Summarizing Large Query Logs in Ettu

Database access logs are large, unwieldy, and hard for humans to inspect and summarize. In spite of this, they remain the canonical go-to resource for tasks ranging from performance tuning to security auditing. In this paper, we address the challenge of compactly encoding large sequences of SQL queries for presentation to a human user. Our approach is based on the Weisfeiler-Lehman (WL) approximate graph isomorphism algorithm, which identifies salient features of a graph or in our case of an abstract syntax tree. Our generalization of WL allows us to define a distance metric for SQL queries, which in turn permits automated clustering of queries. We also present two techniques for visualizing query clusters, and an algorithm that allows these visualizations to be constructed at interactive speeds. Finally, we evaluate our algorithms in the context of a motivating example: insider threat detection at a large US bank. We show experimentally on real world query logs that (a) our distance metric captures a meaningful notion of similarity, and (b) the log summarization process is scalable and performant.

==> Makefile <==
TEX_FILES=paper.tex paper.bib $(wildcard sections/*)

all: paper.pdf todo
	@if [ `uname` = "Darwin" ] ; then open paper.pdf; fi

graphs:
	@cd graphs; rake

paper.pdf: $(TEX_FILES)
	latexmk -pdf paper.tex 

open: paper.pdf todo
	open $<
	
clean:
	latexmk -CA -bibtex

todo:
	@echo "==========================="
	@echo "     Remaining Todos "
	@echo "==========================="
	@find sections -name '*.tex' | \
		xargs grep 'todo' | \
		sed 's:^sections/::; s:\.tex::' | \
		sed 's/\([^:]*\):.*\\todo{/TODO (\1): /; s/}.*//;'


.PHONY: todo plot clean open collabs graphs
